Pretty Good Phone Privacy

To receive service in today's cellular architecture, phones uniquely identify themselves to towers and thus to operators. This is now a cause of major privacy violations, as operators now sell and leak identity and location data of hundreds of millions of mobile users. In this paper, we take an end-to-end perspective on the cellular architecture and find key points of decoupling that enable us to protect user identity and location privacy with no changes to physical infrastructure, no added latency, and no requirement of direct cooperation from existing operators. We describe Pretty Good Phone Privacy (PGPP) and demonstrate how our modified backend stack (NGC) works with real phones to provide ordinary yet privacy-preserving connectivity. We explore inherent privacy and efficiency tradeoffs in a simulation of a large metropolitan region. We show how PGPP maintains today's control overheads while significantly improving user identity and location privacy.

==> sqn.tex <==


\section{Sequence number check}\label{sec:sqn}
When multiple \acrshort{ue}s attach to the network using identical \acrshort{imsi}s, the sequence number check will fail in the network, triggering synch\_failure messages and introducing delay before successful attachment. Figure~\ref{fig:aka} shows the message sequence of the LTE authentication procedure, used today on most celluar networks, and notes what occurs if duplicate IMSIs are present.

When a \acrshort{ue} sends an attach request, the \acrshort{hss} feeds the following to its \acrshort{aka} function: a new nonce value \acrshort{rand}, the shared key K that is stored for the \acrshort{imsi}, and the locally-held sequence number SQN\textsubscript{HSS} for that \acrshort{imsi}. The \acrshort{aka} function generates an authentication token (AUTN\textsubscript{HSS}) that includes the SQN\textsubscript{HSS}, an expected response (\acrshort{xres}), and a key (K\textsubscript{ASME}) that is ultimately used for \acrshort{ue} and \acrshort{mme} authentication. The \acrshort{mme} forwards the \acrshort{rand} and the AUTN\textsubscript{HSS} to the \acrshort{ue}. 

The \acrshort{ue} then uses its own SQN\textsubscript{UE}, its shared key K, and the \acrshort{rand} to generate its own AUTN\textsubscript{UE}, a response (RES), and the key (K\textsubscript{ASME}). The \acrshort{ue} checks if the AUTN\textsubscript{UE} and AUTN\textsubscript{HSS} match and whether the its SQN\textsubscript{UE} matches the SQN\textsubscript{HSS} in the AUTN\textsubscript{HSS}. In PGPP, this will fail for most attach procedures, as individual \acrshort{sim}s will not have the same \acrshort{sqn} value as the \acrshort{hss} for the shared \acrshort{imsi}. When the \acrshort{sqn} check fails the \acrshort{ue} will send an authentication failure message with the cause: \texttt{sync\_failure}, along with the \acrshort{ue}'s current \acrshort{sqn} which allows the \acrshort{hss} to re-synchronize the \acrshort{sqn} value. The \acrshort{ue} then begins the attach sequence again, which will then succeed as the \acrshort{hss} and \acrshort{ue} should begin the attach procedure with the same \acrshort{sqn} values. %We find in our testbed that this works in practice, even with multiple phones attempting to attach simultaneously.

